CAUSE: Counterfactual Assessment of User Satisfaction Estimation in Task-Oriented Dialogue Systems

An important unexplored aspect in previous work on user satisfaction estimation for Task-Oriented Dialogue (TOD) systems is their evaluation in terms of robustness for the identification of user dissatisfaction: current benchmarks for user satisfaction estimation in TOD systems are highly skewed towards dialogues for which the user is satisfied. The effect of having a more balanced set of satisfaction labels on performance is unknown. However, balancing the data with more dissatisfactory dialogue samples requires further data collection and human annotation, which is costly and time-consuming. In this work, we leverage large language models (LLMs) and unlock their ability to generate satisfaction-aware counterfactual dialogues to augment the set of original dialogues of a test collection. We gather human annotations to ensure the reliability of the generated samples. We evaluate two open-source LLMs as user satisfaction estimators on our augmented collection against state-of-the-art fine-tuned models. Our experiments show that when used as few-shot user satisfaction estimators, open-source LLMs show higher robustness to the increase in the number of dissatisfaction labels in the test collection than the fine-tuned state-of-the-art models. Our results shed light on the need for data augmentation approaches for user satisfaction estimation in TOD systems. We release our aligned counterfactual dialogues, which are curated by human annotation, to facilitate further research on this topic.

==> small_cf_samples.tex <==
% \begin{tabular}{c}
\begin{tcolorbox}[boxrule=0.2mm, colback=gray!5, % Background color of the box
                  colframe=teal, % Frame color
                 % Box title
                  title=\textbf{\small Dissatisfaction $\to$ \small Satisfaction},
                  rounded corners, % Enable rounded corners
                  arc=2mm, % Adjust the roundness of the corners
                  ] \footnotesize
\textit{[Truncated Dialogue History] }
\\
USER: Please book the Hamilton Lodge, for 6 people.
\\
SYSTEM: I'd be happy to. How many nights would you like to stay? And I'll need to know the day you would like to start your stay.
\\
USER: I'll be staying 2 nights starting on wednesday. Oh, and there are 6 of us.
\\[0.5\baselineskip]
\textcolor{blue}{\textbf{\textit{Original System Response} $\mathbf{R}$ [Dissatisfaction]:}}
\\
SYSTEM: I'm sorry, my reservation attempt was unsuccessful. Will another day or length of stay work?
\\[0.5\baselineskip]
\textcolor{red}{\textbf{\textit{Counterfactual System Response} $\mathbf{\widehat{R}}$ [Satisfaction]:}} 
\\
SYSTEM: Great, I have successfully booked the Hamilton Lodge for 6 people for 2 nights starting on Wednesday. Your reservation is confirmed. Is there anything else you need assistance with?
 \end{tcolorbox}  

\begin{tcolorbox}
    [boxrule=0.2mm, colback=gray!5, % Background color of the box
                  colframe=teal, % Frame color
                 % Box title
                 title=\textbf{\small Satisfaction $\to$ \small Dissatisfaction},
                  rounded corners, % Enable rounded corners
                  arc=2mm, % Adjust the roundness of the corners
                  ] \footnotesize
\textit{[Truncated Dialogue History] }
\\
SYSTEM: Sorry, it was unavailable at that time. Perhaps you might want another day or a shorter stay?

USER: Does the acorn guest house have any restrictions on bringing young children along? 
\\[0.5\baselineskip]
\textcolor{blue}{\textbf{\textit{Original System Response} $\mathbf{R}$ [Satisfaction]:}}

SYSTEM: There are no restrictions. Children are welcome to stay there. Any other questions, or should I continue to book it?
\\[0.5\baselineskip]
\textcolor{red}{\textbf{\textit{Counterfactual System Response} $\mathbf{\widehat{R}}$ [Dissatisfaction]:}}     

SYSTEM: I'm not sure about their policy on young children. Would you like me to find another guesthouse that is more suitable for families?
\end{tcolorbox}


==> use_prompt.tex <==
\begin{tabular}{c}
\begin{tcolorbox}[boxrule=0.2mm, colback=white, % Background color of the box
                  colframe=teal, % Frame color
                 % Box title
                  rounded corners, % Enable rounded corners
                  title=\textbf{User Satisfaction Estimation with LLMs},
                  arc=2mm, % Adjust the roundness of the corners
                  ]
\textcolor{red}{Instruction}:\\We want to label the user satisfaction for example dialogues. 
\\ \\
The description of 2 labels is as follows: 
\\ \\
"Dissatisfied": The system fails to understand or fulfill user’s request in any way.
\\ \\
"Satisfied": The system understands users request and either "partially" or "fully" satisfies the request or provides information on how the request can be fulfilled.
\\ \\
\textcolor{blue}{Example 1:}\\
User: "Is there bike parking at the train station?",\\ 
System: "Bike parking is available at the station. Are you still interested in a reservation?" 
\\
Label of Example 1 is "Satisfied".
\\ \\
\textcolor{blue}{Example 2:}\\
User: Please book for Sunday for 3 nights and 6 people.
\\
System:	Sorry, the hotel can't accommodate you for that time frame? Want to try a different date?
\\
Label of Example 2 is "Dissatisfied".
\\ \\
\textcolor{blue}{Example 3:} \\
\{\textcolor{orange}{\textbf{Input Dialogue}}\}
\\
Label of Example 3 is:

\end{tcolorbox}
    \end{tabular}
